Chandra/LETGS Studies of the Collisional Plasma in 4U 1626-67

We present an analysis of \chandra/LETGS observations of the ultracompact X-ray binary (UCXB) 4U 1626$-$67, continuing our project to analyze the existing Chandra gratings data of this interesting source. The extremely low mass, hydrogen-depleted donor star provides a unique opportunity to study the properties and structure of the metal-rich accreted plasma. There are strong, double-peaked emission features of OVII-VIII and Ne IX-X, but no other identified emission lines are detected. Our spectral fit simultaneously models the emission line profiles and the plasma parameters, using a two-temperature collisionally-ionized plasma. Based on our line profile fitting, we constrain the inclination of the system to 25--60$^{\circ}$ and the inner disk radius to $\sim$1500 gravitational radii, in turn constraining the donor mass to $\lesssim$0.026 M_sun, while our plasma modeling confirms previous reports of high neon abundance in the source, establishing a Ne/O ratio in the system of $0.47 \pm 0.04$, while simultaneously estimating a very low Fe/O ratio of $0.0042 \pm 0.0008$ and limiting the Mg/O ratio to less than 1% by number. We discuss these results in light of previous work.

==> linelist.tex <==
\begin{deluxetable}{lrrr}
  \tabletypesize{\footnotesize}
  \tablewidth{0pt}
  \tablecaption{All lines with fluxes greater than $10^{-4}$\,ph\,cm$^{-2}$\,s$^{-1}$ \label{tab:linelist}}
  \tablehead{\colhead{Ion} & \colhead{Transition} & \colhead{$\lambda$ (\AA)} & \colhead{Flux\tablenotemark{*}}}
  \startdata
  Ne \textsc{X}   & 3p1 - 1s1                     & 10.238  & 2.286 \\
  Ne \textsc{X}   & 3p1 - 1s1                     & 10.240  & 1.142 \\
  Ne \textsc{X}   & 2p1 - 1s1                     & 12.132  & 15.31 \\
  Ne \textsc{X}   & 2p1 - 1s1                     & 12.137  & 7.651 \\
  Fe \textsc{XXI} & 1s2 2s2 2p1 3d1 - 1s2 2s2 2p2 & 12.284  & 1.562 \\
  Ne \textsc{IX}  & 1s1 2p1 - 1s2                 & 13.447  & 3.146 \\
  Ne \textsc{IX}  & 1s1 2s1 - 1s2                 & 13.699  & 1.734 \\
  O \textsc{VIII} & 3p1 - 1s1                     & 16.006  & 2.631 \\
  O \textsc{VIII} & 3p1 - 1s1                     & 16.007  & 1.314 \\
  O \textsc{VII}  & 1s1 3p1 - 1s2                 & 18.627  & 1.088 \\
  O \textsc{VIII} & 2p1 - 1s1                     & 18.967  & 18.31 \\
  O \textsc{VIII} & 2p1 - 1s1                     & 18.973  & 9.154 \\
  O \textsc{VII}  & 1s1 2p1 - 1s2                 & 21.602  & 8.263 \\
  O \textsc{VII}  & 1s1 2p1 - 1s2                 & 21.804  & 1.371 \\
  O \textsc{VII}  & 1s1 2s1 - 1s2                 & 22.098  & 6.033 \\
  C \textsc{VI}   & 2p1 - 1s1                     & 33.734  & 5.193 \\
  C \textsc{VI}   & 2p1 - 1s1                     & 33.740  & 2.597 \\
  \enddata
  \tablenotetext{*}{Units: $10^{-4}$\,erg\,cm$^{-2}$\,s$^{-1}$}
  % \tablenotetext{\dag}{Overproduced by model spectrum}
\end{deluxetable}

